Enforcing Hard Constraints with Soft Barriers: Safe Reinforcement Learning in Unknown Stochastic Environments

It is quite challenging to ensure the safety of reinforcement learning (RL) agents in an unknown and stochastic environment under hard constraints that require the system state not to reach certain specified unsafe regions. Many popular safe RL methods such as those based on the Constrained Markov Decision Process (CMDP) paradigm formulate safety violations in a cost function and try to constrain the expectation of cumulative cost under a threshold. However, it is often difficult to effectively capture and enforce hard reachability-based safety constraints indirectly with such constraints on safety violation costs. In this work, we leverage the notion of barrier function to explicitly encode the hard safety constraints, and given that the environment is unknown, relax them to our design of \emph{generative-model-based soft barrier functions}. Based on such soft barriers, we propose a safe RL approach that can jointly learn the environment and optimize the control policy, while effectively avoiding unsafe regions with safety probability optimization. Experiments on a set of examples demonstrate that our approach can effectively enforce hard safety constraints and significantly outperform CMDP-based baseline methods in system safe rate measured via simulations.

==> problem_formulation.tex <==
\section{Problem formulation}\label{sec:problem_formulation}

This paper targets to solve the problem of safe policy learning with probabilistic guarantees in the unknown stochastic environment. The environment can be abstracted as a general finite-horizon Markov Decision Process (MDP) $\mathcal{M}$ with tuple $\mathcal{M} \sim(\mathcal{S, A, P}, r, \gamma, \pi)$ where $\mathcal{S} \in \mathbb{R}^n$ represents the continuous state space, $\mathcal{A} \in \mathbb{R}^m$ indicates the continuous action space, $\mathcal{P:S \times A \times S \rightarrow } [0, 1] $ denotes the unknown stochastic environment dynamics, the rewards function $r(s, a) : \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$ is known and the discount factor $\gamma$ $\in [0, 1]$.
A deterministic continuous NN-based policy $\pi_{\theta}: \mathcal{S} \rightarrow \mathcal{A}$ maps the states $s(t) \in \mathcal{S}$  to an action $a(t) \in \mathcal{A}$ at time $t$ as $a(t) = \pi_{\theta}(s(t))$. 
The environment has several known spaces, defined as state space $S \subset \mathcal{S}$, initial space $S_0 \subset \mathcal{S}$, unsafe space $S_u \subset \mathcal{S}$. Without loss of generality, The RL objective is to maximize the total discounted expect return as $\max_{\pi_{\theta}} J := \mathbb{E}_{s(0) \in S_0, P(s'|s, a)  }\left[\sum_{i=0}^{T} \gamma^i r(s(t), a(t))\right]$ with $P \in \mathcal{P}$.

With the above definitions, we can define the probabilistic safety property on the trajectory as
\begin{definition}
(RL Probabilistic Safety Property) For the MDP $\mathcal{M}$ defined above, let $\tau = \{s(0), a(0),  \cdots, s(T), a(T)\} (s(0) \in S_0)$  denotes a sample trajectory from the environment $\mathcal{M}$ with policy $\pi$ and $\tau_t$ is the state $s(t)$ at time $t \in [0, T]$.  Due to the stochasticity in $\mathcal{M}$, state $s$ is a random variable and thus $\tau$ is a random process, then safety probability in RL is defined as 
\begin{displaymath}
\forall t \in [0, T], P(\tau_t \not\in S_u)  \Longrightarrow P(d(\tau_{t}, S_u) > D), \forall  t \in  [0, T]
\end{displaymath}
\end{definition}
where $d(\tau_t, S_u) = \min_{s_u \in S_u} \norm{\tau_t - s_u} $ is a function measuring the minimal distance between trajectory state $\tau_t$ at time $t$ and unsafe region $S_u$ and $D$ is the safety margin. Thus the research problem of safe RL with a probabilistic guarantee can be expressed as 
\begin{problem}
Given an unknown stochastic environment which can be described as an MDP $\mathcal{M}$ defined above, learn a deterministic NN policy $\pi_{\theta}$, such that the system satisfies the safety property with at least probability $1 - \eta \in [0, 1]$ while maximizing the RL objective $J(\pi_{\theta})$ as
\begin{displaymath}
\begin{aligned}
\max_{\pi_{\theta}} J &= \mathbb{E}_{s(0) \in S_0, P(s'|s, a)}\left[\sum_{t=0}^{T} \gamma^t r(s(t), a(t))\right],  \mathrm{s.t.}~~ P(d(\tau_t, S_u) > D) \geq 1 - \eta, \forall t \in [0, T]
\end{aligned}
\end{displaymath}
where $1 - \eta$ is a lower bound of safety probability on the trajectory.
\end{problem}

It is important to clarify the difference between the above formulation and CMDP, as CMDP is expressed as
\begin{displaymath}
\begin{aligned}
\max_{\pi} J &= \mathbb{E}_{s(0) \in S_0, P(s'|s, a)}\left[\sum_{t=0}^{T} \gamma^t r(s(t), a(t))\right], \textrm{s.t.} \ \mathbb{E} \left[\sum_{t=0}^{T}\gamma^t c(\tau_t, S_u)\right] < D'
\end{aligned}
\end{displaymath}
where $c$ is a cost function and $D'$ is total cost budget. The safety constraint in CMDP is weak as it is expressed as an expectation $\mathbb{E}$ of cumulative discounted $\gamma^t$ total cost, while ours are hard safety constraints by the probability bound on every state $\tau_t, \forall t \in [0, T]$.

